WildQA: In-the-Wild Video Question Answering

Existing video understanding datasets mostly focus on human interactions, with little attention being paid to the "in the wild" settings, where the videos are recorded outdoors. We propose WILDQA, a video understanding dataset of videos recorded in outside settings. In addition to video question answering (Video QA), we also introduce the new task of identifying visual support for a given question and answer (Video Evidence Selection). Through evaluations using a wide range of baseline models, we show that WILDQA poses new challenges to the vision and language research communities. The dataset is available at https://lit.eecs.umich.edu/wildqa/.

==> unused/results.tex <==
\begin{table*}[ht!]
\small
 \begin{adjustwidth}{-1.2cm}{}
\begin{tabular}{lrrrrrrr}
 \toprule
 Model name & EM & BLEU\@1 & BLEU\@2 & BLEU\@3 & ROUGE\@1 & ROUGE\@2 & ROUGE\@L \\
 \midrule
 \mn{Random Text}  & 0.36 $\pm$ 0.07 & 5.21 $\pm$ 0.43 & 1.69 $\pm$ 0.38 & 0.46 $\pm$ 0.33 & 5.27 $\pm$ 0.47 & 0.59 $\pm$ 0.25 & 5.11 $\pm$ 0.4 \\
 
 \mn{Most Common Answer}  & 5.52 $\pm$ 0.0 & 0.05 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.64 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.64 $\pm$ 0.0 \\
 
 \mn{Closest Retrieval} & 2.3 $\pm$ 0.0 & 16.31 $\pm$ 0.0 & 8.99 $\pm$ 0.0 & 5.18 $\pm$ 0.0 & 19.5 $\pm$ 0.0 & 6.18 $\pm$ 0.0 & 18.75 $\pm$ 0.0\\
 
 \mn{T5 Zero Shot} & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.84 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.75 $\pm$ 0.0 \\
 
 \mn{T5 Text}  & 3.27 $\pm$ 0.44 & 30.44 $\pm$ 0.09 & 23.33 $\pm$ 0.1 & 18.99 $\pm$ 0.1 & 34.65 $\pm$ 0.82 & 18.18 $\pm$ 0.39 & 33.22 $\pm$ 0.75 \\
 
 \mn{T5 Text + Visual} & 3.02 $\pm$ 0.07 & 29.9 $\pm$ 0.5 & 22.71 $\pm$ 0.34 & 18.42 $\pm$ 0.24 & 34.04 $\pm$ 0.58 & 17.76 $\pm$ 0.26 & 32.66 $\pm$ 0.5  \\
 
 \mn{CLIP + T5 Decoder} & 1.23 $\pm$ 0.25 & 14.04 $\pm$ 1.72 & 7.84 $\pm$ 1.35 & 4.58 $\pm$ 0.87 & 16.89 $\pm$ 2.46 & 5.23 $\pm$ 1.06 & 16.29 $\pm$ 2.37 \\
 
 \mn{CLIP + T5 Decoder}$_\text{TVQA}$ & 1.48 $\pm$ 0.59 & 12.13 $\pm$ 0.95 & 6.74 $\pm$ 0.57 & 3.73 $\pm$ 0.31 & 15.60 $\pm$ 0.51 & 4.56 $\pm$ 0.46 & 15.11 $\pm$ 0.42 \\
 
 \mn{Multi-Task} & 3.37 $\pm$ 0.33 & 28.78 $\pm$ 0.43 & 21.85 $\pm$ 0.43 & 17.74 $\pm$ 0.41 & 33.53 $\pm$ 0.57 & 17.06 $\pm$ 0.53 & 32.18 $\pm$ 0.51 \\
 \bottomrule
\end{tabular}
   \end{adjustwidth}
\caption{Baseline results for few-shot experiments for 15 epochs}
\label{tab: few-shot-qa-results-15-epochs}
\end{table*}

\begin{table*}[ht!]
\small
 \begin{adjustwidth}{-1.2cm}{}
\begin{tabular}{lrrrrrrr}
 \toprule
 Model name & EM & BLEU\@1 & BLEU\@2 & BLEU\@3 & ROUGE\@1 & ROUGE\@2 & ROUGE\@L \\
 \midrule
 \mn{Random Text}  & 0.36 $\pm$ 0.07 & 5.21 $\pm$ 0.43 & 1.69 $\pm$ 0.38 & 0.46 $\pm$ 0.33 & 5.27 $\pm$ 0.47 & 0.59 $\pm$ 0.25 & 5.11 $\pm$ 0.40 \\
 
 \mn{Most Common Answer}  & 5.52 $\pm$ 0.00 & 0.05 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.0 & 10.64 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 10.64 $\pm$ 0.00 \\
 
 \mn{Closest Retrieval} & 2.3 $\pm$ 0.00 & 16.31 $\pm$ 0.00 & 8.99 $\pm$ 0.00 & 5.18 $\pm$ 0.00 & 19.5 $\pm$ 0.00 & 6.18 $\pm$ 0.00 & 18.75 $\pm$ 0.00\\
 
 \mn{T5 Zero Shot} & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.84 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.75 $\pm$ 0.00 \\
 
 \mn{T5 Text}   & 3.22 $\pm$ 0.33 & 28.98 $\pm$ 0.08 & 22.26 $\pm$ 0.12 & 18.21 $\pm$ 0.11 & 34.08 $\pm$ 0.81 & 17.62 $\pm$ 0.05 & 32.81 $\pm$ 0.78 \\
 
 \mn{T5 Text + Visual} & 2.81 $\pm$ 0.29 & 29.32 $\pm$ 0.52 & 22.35 $\pm$ 0.36 & 18.09 $\pm$ 0.26 & 33.27 $\pm$ 0.39 & 17.38 $\pm$ 0.38 & 32.03 $\pm$ 0.33  \\
 
 \mn{CLIP + T5 Decoder} & 0.92 $\pm$ 0.45 & 12.99 $\pm$ 2.36 & 7.43 $\pm$ 1.66 & 4.39 $\pm$ 1.12 & 15.83 $\pm$ 3.61 & 5.28 $\pm$ 1.42 & 15.45 $\pm$ 3.49 \\
 
 \mn{CLIP + T5 Decoder}$_\text{TVQA}$ & 0.77 $\pm$ 0.00 & 12.1 $\pm$ 1.61 & 6.54 $\pm$ 1.14 & 3.64 $\pm$ 0.79 & 14.85 $\pm$ 2.17 & 4.37 $\pm$ 1.04 & 14.43 $\pm$ 2.04 \\
 
 \mn{Multi-Task} & 2.91 $\pm$ 0.33 & 29.23 $\pm$ 0.40 & 22.30 $\pm$ 0.23 & 18.12 $\pm$ 0.38 & 33.70 $\pm$ 0.45 & 17.63 $\pm$ 0.52 & 32.40 $\pm$ 0.49 \\
 \bottomrule
\end{tabular}
\end{adjustwidth}
\caption{Baseline results for few-shot experiments for 20 epochs}
\label{tab: few-shot-qa-results-20-epochs}
\end{table*}

\begin{table}[ht!]
\begin{tabular}{lr}
 \toprule
 Model name & IOU-F1 \\
 \midrule
\mn{Random Evidence} & 18.52 $\pm$ 0.14 \\

\mn{T5 Start End} & 24.25 $\pm$ 6.20 \\

\mn{T5 IO}  & 26.74 $\pm$ 0.11 \\

\mn{Multi-Task}   & 27.48 $\pm$ 3.62 \\
 \bottomrule
\end{tabular}
\caption{Baseline results for few-shot experiments for 15 epochs}
\label{tab: few-shot-evidence-results-15-epochs}
\end{table}

\begin{table}[ht!]
\begin{tabular}{lr}
 \toprule
 Model name & IOU-F1 \\
 \midrule
\mn{Random Evidence} & 18.52 $\pm$ 0.14 \\

\mn{T5 Start End} & 21.77 $\pm$ 1.30 \\

\mn{T5 IO} & 26.81 $\pm$ 0.52 \\

\mn{Multi-Task}   & 20.77 $\pm$ 2.14 \\
 \bottomrule
\end{tabular}
\caption{Baseline results for few-shot experiments for 15 epochs}
\label{tab: few-shot-evidence-results-15-epochs}
\end{table}

% with exact match

\begin{table*}[ht!]
\small
\begin{tabular}{lrrrrrrr}
 \toprule
 Model name & EM & BLEU\@1 & BLEU\@2 & BLEU\@3 & ROUGE\@1 & ROUGE\@2 & ROUGE\@L \\
 \midrule
 \mn{Random Text}  & 5.5 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 \\
 
 \mn{Most Common}   & 5.5 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0  \\
 
 \mn{Closest Rtr}  & 2.3 $\pm$ 0.0 & 16.3 $\pm$ 0.0 & 9.0 $\pm$ 0.0 & 5.2 $\pm$ 0.0 & 19.5 $\pm$ 0.0 & 6.2 $\pm$ 0.0 & 18.7 $\pm$ 0.0 \\
 
\hdashline

 \mn{T5 Zero Shot} & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 \\
 
 \mn{T5 Text} & 3.0 $\pm$ 0.1 & 29.6 $\pm$ 0.2 & 22.6 $\pm$ 0.2 & 18.5 $\pm$ 0.1 & 33.8 $\pm$ 0.2 & 17.7 $\pm$ 0.1 & 32.4 $\pm$ 0.3 \\
 
 \mn{T5 T + V}  & 2.7 $\pm$ 0.4 & 29.5 $\pm$ 0.5 & 22.5 $\pm$ 0.4 & 18.2 $\pm$ 0.3 & 33.1 $\pm$ 0.3 & 17.3 $\pm$ 0.4 & 31.9 $\pm$ 0.2  \\
 
  \mn{Multi-Task} & 3.0 $\pm$ 0.5 & 29.6 $\pm$ 0.9 & 22.5 $\pm$ 0.9 & 18.3 $\pm$ 1.0 & 33.2 $\pm$ 1.5 & 17.6 $\pm$ 0.8 & 31.8 $\pm$ 1.5 \\
  
  \hdashline
 
 \mn{CLIP + D$_\text{T5}$}  & 1.0 $\pm$ 0.6 & 10.9 $\pm$ 0.2 & 5.7 $\pm$ 0.4 & 2.9 $\pm$ 0.3 & 14.1 $\pm$ 1.2 & 3.6 $\pm$ 0.4 & 13.7 $\pm$ 1.2 \\
 
 \mn{CLIP + D$_\text{T5}$}$_\text{TVQA}$ & 0.6 $\pm$ 0.1 & 7.0 $\pm$ 4.5 & 4.0 $\pm$ 2.4 & 2.1 $\pm$ 1.1 & 13.2 $\pm$ 1.8 & 3.7 $\pm$ 0.3 & 13.0 $\pm$ 1.8 \\
 
 \bottomrule
\end{tabular}
\caption{Baseline results for few-shot experiments for 10 epochs}
\label{tab: few-shot-qa-results-10-epochs}
\end{table*}

\begin{table*}[ht!]

\begin{tabular}{lrrrrrr}
 \toprule
 Model name  & BLEU\@1 & BLEU\@2 & BLEU\@3 & ROUGE\@1 & ROUGE\@2 & ROUGE\@L \\
 \midrule
 \mn{Random Text}   & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 \\
 
 \mn{Most Common}   & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0  \\
 
 \mn{Closest Rtr}  & 16.3 $\pm$ 0.0 & 9.0 $\pm$ 0.0 & 5.2 $\pm$ 0.0 & 19.5 $\pm$ 0.0 & 6.2 $\pm$ 0.0 & 18.7 $\pm$ 0.0 \\
 
\hdashline

 \mn{T5 Zero Shot} & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 \\
 
 \mn{T5 Text} & 29.6 $\pm$ 0.2 & 22.6 $\pm$ 0.2 & 18.5 $\pm$ 0.1 & 33.8 $\pm$ 0.2 & 17.7 $\pm$ 0.1 & 32.4 $\pm$ 0.3 \\
 
 \mn{T5 T + V}  & 29.5 $\pm$ 0.5 & 22.5 $\pm$ 0.4 & 18.2 $\pm$ 0.3 & 33.1 $\pm$ 0.3 & 17.3 $\pm$ 0.4 & 31.9 $\pm$ 0.2  \\
 
 \mn{Multi-Task}  & 29.6 $\pm$ 0.9 & 22.5 $\pm$ 0.9 & 18.3 $\pm$ 1.0 & 33.2 $\pm$ 1.5 & 17.6 $\pm$ 0.8 & 31.8 $\pm$ 1.5 \\
  
  \hdashline
 
 \mn{CLIP + D$_\text{T5}$}  & 10.9 $\pm$ 0.2 & 5.7 $\pm$ 0.4 & 2.9 $\pm$ 0.3 & 14.1 $\pm$ 1.2 & 3.6 $\pm$ 0.4 & 13.7 $\pm$ 1.2 \\
 
 \mn{CLIP + D$_\text{T5}$}$_\text{TVQA}$  & 7.0 $\pm$ 4.5 & 4.0 $\pm$ 2.4 & 2.1 $\pm$ 1.1 & 13.2 $\pm$ 1.8 & 3.7 $\pm$ 0.3 & 13.0 $\pm$ 1.8 \\
 
 \bottomrule
\end{tabular}
\caption{Baseline results for few-shot experiments for 10 epochs}
\label{tab: few-shot-qa-results-10-epochs}
\end{table*}



\begin{figure}[ht!]
\centering
\includegraphics{figures/model-performance/baseline-performance-evidence-cropped.pdf}
\caption{Performance comparison between .}
\label{fig: model-performance-evidence}
\end{figure}


% Baseline performanceon Video QA with exact match

\begin{table*}[ht!]
\small
\begin{tabular}{lrrrrrrr}
 \toprule
 Model name & EM & BLEU\@1 & BLEU\@2 & BLEU\@3 & ROUGE\@1 & ROUGE\@2 & ROUGE\@L \\
 \midrule
 \mn{Random Text}  & 5.5 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 \\
 
 \mn{Most Common}   & 5.5 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0  \\
 
 \mn{Closest Rtr}  & 2.3 $\pm$ 0.0 & 16.3 $\pm$ 0.0 & 9.0 $\pm$ 0.0 & 5.2 $\pm$ 0.0 & 19.5 $\pm$ 0.0 & 6.2 $\pm$ 0.0 & 18.7 $\pm$ 0.0 \\
 
\hdashline

 \mn{T5 Zero Shot} & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 \\
 
 \mn{T5 Text} & \textbf{3.0 $\pm$ 0.1} & \textbf{29.6 $\pm$ 0.2} & \textbf{22.6 $\pm$ 0.2} & \textbf{18.5 $\pm$ 0.1} & \textbf{33.8 $\pm$ 0.2} & \textbf{17.7 $\pm$ 0.1} & \textbf{32.4 $\pm$ 0.3} \\
 
 \mn{T5 T + V}  & 2.7 $\pm$ 0.4 & 29.5 $\pm$ 0.5 & 22.5 $\pm$ 0.4 & 18.2 $\pm$ 0.3 & 33.1 $\pm$ 0.3 & 17.3 $\pm$ 0.4 & 31.9 $\pm$ 0.2  \\
 
  \mn{Multi-Task} & \textbf{3.0 $\pm$ 0.5} & \textbf{29.6 $\pm$ 0.9} & \textbf{22.5 $\pm$ 0.9} & \textbf{18.3 $\pm$ 1.0} & \textbf{33.2 $\pm$ 1.5} & \textbf{17.6 $\pm$ 0.8} & \textbf{31.8 $\pm$ 1.5} \\
 \bottomrule
\end{tabular}
\caption{Baseline results for Video Question Answering experiments. ``EM'' represents exact match scores. For comparison, we also test the out-of-box T5 model on our testing split in a zero-shot fashion (\mn{T5 Zero Shot}). We run each model 3 times and report the mean $\pm$ standard deviation scores.}
\label{tab: few-shot-qa-results-10-epochs}
\end{table*}

% With BLEU and ROUGE scores 

\begin{table*}[ht!]
\small
\begin{tabular}{lrrrrrr}
 \toprule
 Model name  & B\@1 & B\@2 & B\@3 & R\@1 & R\@2 & R\@L \\
 \midrule
 \mn{Random Text}  &4.9 $\pm$ 0.2&1.6 $\pm$ 0.3&0.5 $\pm$ 0.4&5.0 $\pm$ 0.2&0.5 $\pm$ 0.1&4.9 $\pm$ 0.2\\
 
 \mn{Most Common}   & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 10.6 $\pm$ 0.0  \\
 
 \mn{Closest Rtr}   & 16.3 $\pm$ 0.0 & 9.0 $\pm$ 0.0 & 5.2 $\pm$ 0.0 & 19.5 $\pm$ 0.0 & 6.2 $\pm$ 0.0 & 18.7 $\pm$ 0.0 \\
 
\hdashline

 \mn{T5 Text$^\text{zero shot}$}  & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 \\
 
 \mn{T5 Text}  & 29.6 $\pm$ 0.2& 22.6 $\pm$ 0.2& 18.5 $\pm$ 0.1& 33.8 $\pm$ 0.2& 17.7 $\pm$ 0.1& 32.4 $\pm$ 0.3 \\
 
 \mn{T5 T + V}  & 29.5 $\pm$ 0.5 & 22.5 $\pm$ 0.4 & 18.2 $\pm$ 0.3 & 33.1 $\pm$ 0.3 & 17.3 $\pm$ 0.4 & 31.9 $\pm$ 0.2  \\

  \mn{Multi$_\text{T+V,IO}$} &\textbf{30.5} $\pm$ \textbf{0.6}&\textbf{23.6} $\pm$ \textbf{0.7}&\textbf{19.3} $\pm$ \textbf{0.8}&\textbf{34.0} $\pm$ \textbf{0.5}&\textbf{18.8} $\pm$ \textbf{0.7}&\textbf{32.8} $\pm$ \textbf{0.6}\\
  
  \mn{Multi$_\text{T+V,SE}$} &30.2 $\pm$ 0.8&23.2 $\pm$ 0.7&18.9 $\pm$ 0.6&33.8 $\pm$ 0.8&18.5 $\pm$ 0.7&32.5 $\pm$ 0.8\\
  
  \midrule 
  \mn{Human} & 44.3 $\pm$ 0.0 & 17.0 $\pm$ 0.0 & 8.2 $\pm$ 0.0 & 42.1 $\pm$ 0.0 & 19.4 $\pm$ 0.0 & 37.8 $\pm$ 0.0 \\
 \bottomrule
\end{tabular}
\caption{BLEU and ROUGE scores for the task of Video Question Answering. For comparison, we also test the out-of-box T5 model on our testing split in a zero-shot fashion (\mn{T5 Zero Shot}).}
\label{tab: few-shot-qa-results-10-epochs}
\end{table*}



%  IOU-F1 scores on different question types
\begin{table}[t!]
\begin{tabular}{lr}
 \toprule
 Type & IOU-F1 \\
 \midrule
Entity& 21.3 $\pm$ 8.0 \\
Reasoning& 38.1 $\pm$ 8.9 \\
Location& 28.4 $\pm$ 15.5 \\
Motion& 38.1 $\pm$ 3.4 \\
Spatial& 31.0 $\pm$ 3.4 \\
Other& 45.2 $\pm$ 6.7 \\
Number& 31.0 $\pm$ 3.4 \\
Existence& 26.0 $\pm$ 4.9 \\
Time& 21.4 $\pm$ 0.0 \\
Temporal& 35.7 $\pm$ 5.8 \\
 \bottomrule
\end{tabular}
\caption{\mn{Multi-Task} performance on different question types for Video Evidence Selection}
\label{tab: type-performance}
\end{table}
